Feature Based Task Recommendation in Crowdsourcing with Implicit Observations

Existing research in crowdsourcing has investigated how to recommend tasks to workers based on which task the workers have already completed, referred to as {\em implicit feedback}. We, on the other hand, investigate the task recommendation problem, where we leverage both implicit feedback and explicit features of the task. We assume that we are given a set of workers, a set of tasks, interactions (such as the number of times a worker has completed a particular task), and the presence of explicit features of each task (such as, task location). We intend to recommend tasks to the workers by exploiting the implicit interactions, and the presence or absence of explicit features in the tasks. We formalize the problem as an optimization problem, propose two alternative problem formulations and respective solutions that exploit implicit feedback, explicit features, as well as similarity between the tasks. We compare the efficacy of our proposed solutions against multiple state-of-the-art techniques using two large scale real world datasets.

==> algorithms.tex <==
\section{Algorithms for Task Recommendations}
\label{sec:algorithms}
%{\bf I will come back to the section later if I get time}
In this section, we present our solutions based on the two alternative formulations described in previous section.

\subsection{Solution using Feature Preference Model }\label{sec:algorithms}
In this section we present the techniques to solve the objective function described in Equation~\ref{eqn:objective}. Throughout the following sections we refer to our algorithms as \\{\tt Feature-Based-NNLS} or Feature Based Non-Negative-Least Square . Here, we have a fixed  $Y$ matrix and the non-negativity of matrix $X$ needs to be respected. Since $Y$ matrix is fixed in our case, the objective function is quadratic. 

In order to solve for $X$ by minimizing the objective function described in Equation~\ref{eqn:objective}, first we need to take the derivative against each user vector $x_u$. Let's introduce another notation $W_u$ which denotes a diagonal matrix, where $W^u_{ii} = w_{ui}$.

\begin{align*}
\frac{\partial M}{\partial x_u} &= -2\sum_iw_{ui}(p_{ui}-{x_u^Ty_i})y_i+2\lambda x_u\\
&= -2Y^tW^up_u + 2Y^tW^uYx_u + 2 \lambda x_u
\end{align*}

Now, by putting $\frac{\partial M}{\partial x_u} = 0$ we get the analytical solution for $x_u$ as - 

\begin{align}
\label{eqn:user}
x_u =  (Y^tW^uY + \lambda I)^{-1}Y^tW^uP_u
\end{align}

However, we cannot solve exactly due to the non-negativity constraint. Hence we want to minimize the L-2 error for each user $\|(Y^tW^uY + \lambda I)x_u - Y^tC^uP_u\|^2$. There exists two ways to solve this problem - i) the constrained version of this problem can be transformed using a new formulation to  an unconstrained version and then solve it ii) or, the problem can be solved by treating as a Generalized Singular Value Decomposition problem~\cite{bjorck1996numerical}   

{\bf Complexity :} The worst case complexity for solving this constrained version of the least square problem for each user is  $O(n_l^3)$ since the size of the coefficient matrix in our case is $n_l \times n_l$ ~\cite{bjorck1996numerical}. Hence for each user the complexity becomes $O(n_un_l^3)$. 

% 
% \eat{\subsection{Discussion:} Throughout the previous section, we assume that we know the presence of feature for the task. We present here  two variants of the similar problem- 
% }
\noindent{\bf Presence of User-Feature:} The first variant appears where we know the user's feature preference instead of task feature information. Then, we can use the similar formulation to find out the Task Feature-matrix and thereby solving the task recommendation problem. 

\noindent{\bf Presence of both User-Feature and Task-Feature:} Another variant of this problem appears, when we know only the zero entries of both Task-Feature matrix $Y$ and User-Feature matrix $X$, then the non-zero entries of both matrices are subject to optimization. This problem is similar to solving a sparse constrained matrix factorization problem. This can be computationally expensive if the number of explicit features are too many.

\subsection{Solution using Latent Factor Model}

In this section, we describe the techniques to solve the objective function described in Equation~\ref{eqn:objective2}. We call this algorithm as Implicit Factorization with Task Similarity, \texttt{IFTS}. We apply alternating least square based approach to solve this problem. This is an iterative approach where we partially differentiate objective $M$ with respect to both users and items. At each iteration, we fix the item's latent factor matrix $V$ in order to solve for $U$ and vice versa. If we differentiate the objective function with respect to $U$, we get the similar solution as equation~\ref{eqn:user} for solving $U$, 

\begin{align}
 \label{eqn:user_latent}
 u_u =  (V^tW^uV + \lambda I)^{-1}V^tW^uP_u
\end{align}

However, for solving $V$ we need to consider the penalty term while differentiating against $V$ 
\begin{align*}
\frac{\partial M}{\partial v_i} &= -2\sum_iw_{ui}(p_{ui}-{u_u^Tv_i})v_i+2\lambda v_i -  \lambda\sum_{i'=1}^{n_t}Sim(i,i')v_i' \\
&= -2V^tW^ip_i + 2U^tW^iUv_i + 2 \lambda v_i -  \lambda\sum_{i'=1}^{n_t}Sim(i,i')v_i'\\
\end{align*}

By setting $\frac{\partial M}{\partial v_i}$ = $0$, we get the following equation for solving $v_i$
\begin{align}
  \label{eqn:item_latent}
v_i =  (U^tW^iU + \lambda I)^{-1}(U^tW^iP_i + \lambda * 0.5 * \sum_{i'=1}^{n_t} Sim(i,i')v_i') 
\end{align}

We achieve reasonable speed-up by using the fact that $U^tW_iU$ = $U^tU + U^t(W_i - I)U$~\cite{hu2008collaborative} . We can compute $U^tU$ once and reuse it over all the iterations and number of non-zero elements in $W_i - I$ is exactly the number of users for which $c_{ui} > 0$, let's call that $m_i$, is much smaller than the total number of users. Then, $m << n_u$. The running time of this algorithm is $O(n_f^2\mathbf{N} + n_f^3)$ with the additional cost of  $\sum_{i'=1}^{n_t} Sim(i,i')v_i'$, where $\mathbf{N}$ is the total number of non-zero entries, $\sum_{i=1}^{i=n_t}m_i = \mathbf{N}$. So the overall running time of this algorithm is $O(n_f^2\mathbf{N} + n_f^3 + n_u*n_t)$.  

 
